LLaMA-Excitor: General Instruction Tuning via Indirect Feature Interaction

Existing methods to fine-tune LLMs, like Adapter, Prefix-tuning, and LoRA, which introduce extra modules or additional input sequences to inject new skills or knowledge, may compromise the innate abilities of LLMs. In this paper, we propose LLaMA-Excitor, a lightweight method that stimulates the LLMs' potential to better follow instructions by gradually paying more attention to worthwhile information. Specifically, the LLaMA-Excitor does not directly change the intermediate hidden state during the self-attention calculation of the transformer structure. We designed the Excitor block as a bypass module for the similarity score computation in LLMs' self-attention to reconstruct keys and change the importance of values by learnable prompts. LLaMA-Excitor ensures a self-adaptive allocation of additional attention to input instructions, thus effectively preserving LLMs' pre-trained knowledge when fine-tuning LLMs on low-quality instruction-following datasets. Furthermore, we unify the modeling of multi-modal tuning and language-only tuning, extending LLaMA-Excitor to a powerful visual instruction follower without the need for complex multi-modal alignment. Our proposed approach is evaluated in language-only and multi-modal tuning experimental scenarios. Notably, LLaMA-Excitor is the only method that maintains basic capabilities while achieving a significant improvement (+6%) on the MMLU benchmark. In the visual instruction tuning, we achieve a new state-of-the-art image captioning performance of 157.5 CIDEr on MSCOCO, and a comparable performance (88.39%) on ScienceQA to cutting-edge models with more parameters and extensive vision-language pertaining.

==> tabs/mmlu-full.tex <==
\begin{table*}[h]
\tiny
\centering
\resizebox{0.92\linewidth}{!}{

\begin{tabular}{l|cccc|c}
\toprule
Task	&LLaMA-7B	&LLaMA-full	&LLaMA-lora	&LLaMA-adapter	&LLaMA-Excitor\\
\midrule
high\_school\_statistics	&0.3056 	&0.3194 	&0.2130 	&0.2176 	&0.2546 \\
professional\_medicine	&0.4375 	&0.1985 	&0.4485 	&0.4301 	&0.4301 \\
college\_physics	&0.2353 	&0.1765 	&0.1961 	&0.2451 	&0.2843 \\
college\_chemistry	&0.2800 	&0.2200 	&0.3300 	&0.2700 	&0.3000 \\
global\_facts	&0.3000 	&0.3100 	&0.3300 	&0.3200 	&0.3700 \\
jurisprudence	&0.4167 	&0.3519 	&0.3611 	&0.3704 	&0.3889 \\
conceptual\_physics	&0.3660 	&0.2979 	&0.3532 	&0.3830 	&0.3660 \\
machine\_learning	&0.2679 	&0.2321 	&0.3482 	&0.3571 	&0.2679 \\
high\_school\_world\_history	&0.4262 	&0.3333 	&0.4008 	&0.3840 	&0.4177 \\
business\_ethics	&0.4100 	&0.3400 	&0.4300 	&0.3700 	&0.3900 \\
formal\_logic	&0.2540 	&0.1667 	&0.2778 	&0.2460 	&0.2381 \\
high\_school\_mathematics	&0.2630 	&0.2704 	&0.2407 	&0.2407 	&0.2704 \\
management	&0.3398 	&0.3592 	&0.4078 	&0.3689 	&0.3495 \\
world\_religions	&0.4912 	&0.3626 	&0.3918 	&0.4678 	&0.4854 \\
high\_school\_chemistry	&0.2956 	&0.3596 	&0.2956 	&0.2709 	&0.2315 \\
moral\_disputes	&0.3931 	&0.3728 	&0.3353 	&0.3006 	&0.3613 \\
clinical\_knowledge	&0.3623 	&0.4113 	&0.3849 	&0.3962 	&0.4000 \\
high\_school\_physics	&0.2715 	&0.2450 	&0.2318 	&0.2583 	&0.3046 \\
college\_biology	&0.3819 	&0.2847 	&0.3056 	&0.3333 	&0.3333 \\
human\_aging	&0.3991 	&0.3587 	&0.3991 	&0.4170 	&0.4126 \\
professional\_psychology	&0.3562 	&0.3186 	&0.3284 	&0.3023 	&0.3529 \\
computer\_security	&0.4500 	&0.3800 	&0.3900 	&0.4100 	&0.4400 \\
abstract\_algebra	&0.2700 	&0.3400 	&0.2700 	&0.2600 	&0.3000 \\
high\_school\_us\_history	&0.3627 	&0.3235 	&0.3333 	&0.3088 	&0.3431 \\
logical\_fallacies	&0.4233 	&0.2883 	&0.3129 	&0.3681 	&0.3742 \\
elementary\_mathematics	&0.2619 	&0.2778 	&0.2884 	&0.2646 	&0.2540 \\
medical\_genetics	&0.3700 	&0.3300 	&0.3100 	&0.4400 	&0.4200 \\
high\_school\_psychology	&0.4752 	&0.4128 	&0.3872 	&0.4385 	&0.4587 \\
us\_foreign\_policy	&0.4300 	&0.3500 	&0.3800 	&0.4400 	&0.4600 \\
high\_school\_computer\_science	&0.3300 	&0.3400 	&0.3500 	&0.2800 	&0.3000 \\
econometrics	&0.2632 	&0.2632 	&0.2719 	&0.2719 	&0.2544 \\
high\_school\_european\_history	&0.4364 	&0.3394 	&0.3273 	&0.3273 	&0.4182 \\
astronomy	&0.3487 	&0.3553 	&0.3092 	&0.2829 	&0.3618 \\
college\_computer\_science	&0.3200 	&0.2500 	&0.3000 	&0.2900 	&0.2600 \\
human\_sexuality	&0.3435 	&0.3359 	&0.3969 	&0.3282 	&0.4122 \\
public\_relations	&0.4364 	&0.2727 	&0.3636 	&0.4727 	&0.3727 \\
international\_law	&0.5207 	&0.4545 	&0.3802 	&0.5372 	&0.4628 \\
college\_mathematics	&0.3400 	&0.2500 	&0.2900 	&0.3000 	&0.3300 \\
marketing	&0.4701 	&0.4231 	&0.3932 	&0.4487 	&0.5043 \\
sociology	&0.4677 	&0.4726 	&0.3383 	&0.3582 	&0.4726 \\
electrical\_engineering	&0.2414 	&0.2966 	&0.2621 	&0.2690 	&0.2759 \\
nutrition	&0.3856 	&0.3301 	&0.3758 	&0.3954 	&0.3954 \\
professional\_accounting	&0.2589 	&0.2518 	&0.2518 	&0.2482 	&0.2837 \\
security\_studies	&0.3347 	&0.4286 	&0.3265 	&0.2449 	&0.2816 \\
virology	&0.3373 	&0.3735 	&0.3916 	&0.3253 	&0.2831 \\
high\_school\_biology	&0.3387 	&0.2710 	&0.3194 	&0.3161 	&0.4000 \\
high\_school\_macroeconomics	&0.3410 	&0.3154 	&0.3000 	&0.3179 	&0.3564 \\
prehistory	&0.3457 	&0.3488 	&0.2901 	&0.3457 	&0.3981 \\
professional\_law	&0.2979 	&0.2868 	&0.2771 	&0.2608 	&0.2855 \\
college\_medicine	&0.3295 	&0.2486 	&0.3295 	&0.3295 	&0.3642 \\
miscellaneous	&0.4266 	&0.4432 	&0.3883 	&0.4215 	&0.4815 \\
moral\_scenarios	&0.2425 	&0.2469 	&0.2447 	&0.2425 	&0.2425 \\
philosophy	&0.3955 	&0.4019 	&0.3248 	&0.3119 	&0.3505 \\
high\_school\_geography	&0.3232 	&0.4192 	&0.3586 	&0.3232 	&0.3889 \\
anatomy	&0.3852 	&0.3333 	&0.3111 	&0.4000 	&0.3630 \\
high\_school\_government\_and\_politics	&0.4456 	&0.4560 	&0.3886 	&0.3627 	&0.4663 \\
high\_school\_microeconomics	&0.3319 	&0.2521 	&0.3319 	&0.2773 	&0.3529 \\
\midrule
MEAN	&0.3467 	&0.3237 	&0.3311 	&0.3363 	&\textbf{0.3575} \\
\bottomrule
\end{tabular}

}
\caption{Performances on Massive Multitask Language Understanding tasks (MMLU) under the 5-shot in-context-learning setting.}
\label{tabel:MMLU}
\end{table*}

==> tabs/mmlu.tex <==
\begin{table*}[H]
\huge
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{| l | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r | r |} 
\hline
    \rotatebox{90}{ ~~~~~~~~~~~~~~~~~~~~~\textbf{Model}} & \rotatebox{90}{high-school-statistics} & \rotatebox{90}{professional-medicine} & \rotatebox{90}{college-physics} & \rotatebox{90}{college-chemistry} & \rotatebox{90}{global-facts} & \rotatebox{90}{jurisprudence} & \rotatebox{90}{conceptual-physics} & \rotatebox{90}{machine-learning} & \rotatebox{90}{high-school-world-history} & \rotatebox{90}{business-ethics} & \rotatebox{90}{formal-logic} & \rotatebox{90}{high-school-mathematics} & \rotatebox{90}{management} & \rotatebox{90}{world-religions} & \rotatebox{90}{high-school-chemistry} & \rotatebox{90}{moral-disputes} & \rotatebox{90}{clinical-knowledge} & \rotatebox{90}{high-school-physics} & \rotatebox{90}{college-biology} & \rotatebox{90}{human-aging} & \rotatebox{90}{professional-psychology} & \rotatebox{90}{computer-security} & \rotatebox{90}{abstract-algebra} & \rotatebox{90}{high-school-us-history} & \rotatebox{90}{logical-fallacies} & \rotatebox{90}{elementary-mathematics} & \rotatebox{90}{medical-genetics} & \rotatebox{90}{high-school-psychology} & \rotatebox{90}{us-foreign-policy} & \rotatebox{90}{high-school-computer-science} & \rotatebox{90}{econometrics} & \rotatebox{90}{high-school-european-history} & \rotatebox{90}{astronomy} & \rotatebox{90}{college-computer-science} & \rotatebox{90}{human-sexuality} & \rotatebox{90}{public-relations} & \rotatebox{90}{international-law} & \rotatebox{90}{college-mathematics} & \rotatebox{90}{marketing} & \rotatebox{90}{sociology} & \rotatebox{90}{electrical-engineering} & \rotatebox{90}{nutrition} & \rotatebox{90}{professional-accounting} & \rotatebox{90}{security-studies} & \rotatebox{90}{virology} & \rotatebox{90}{high-school-biology} & \rotatebox{90}{high-school-macroeconomics} & \rotatebox{90}{prehistory} & \rotatebox{90}{professional-law} & \rotatebox{90}{college-medicine} & \rotatebox{90}{miscellaneous} & \rotatebox{90}{moral-scenarios} & \rotatebox{90}{philosophy} & \rotatebox{90}{high-school-geography} & \rotatebox{90}{anatomy} & \rotatebox{90}{high-school-government-and-politics} & \rotatebox{90}{high-school-microeconomics} & \rotatebox{90}{~~~~~~~~~~~~~~~~~~~~~\textbf{MEAN}}\\ \hline
    \hline

    \rotatebox{90}{\textbf{LLaMA-7B}       } & \rotatebox{90}{30.56±3.14            } & \rotatebox{90}{30.56±3.14           } & \rotatebox{90}{43.75±3.01     } & \rotatebox{90}{43.75±3.01       } & \rotatebox{90}{23.53±4.22  } & \rotatebox{90}{23.53±4.22   } & \rotatebox{90}{28.00±4.51        } & \rotatebox{90}{28.00±4.51      } & \rotatebox{90}{30.00±4.61               } & \rotatebox{90}{30.00±4.61     } & \rotatebox{90}{41.67±4.77  } & \rotatebox{90}{41.67±4.77             } & \rotatebox{90}{36.60±3.15} & \rotatebox{90}{36.60±3.15     } & \rotatebox{90}{26.79±4.20           } & \rotatebox{90}{26.79±4.20    } & \rotatebox{90}{42.62±3.22        } & \rotatebox{90}{42.62±3.22         } & \rotatebox{90}{41.00±4.94     } & \rotatebox{90}{41.00±4.94 } & \rotatebox{90}{25.40±3.89             } & \rotatebox{90}{25.40±3.89       } & \rotatebox{90}{26.30±2.68      } & \rotatebox{90}{26.30±2.68            } & \rotatebox{90}{33.98±4.69       } & \rotatebox{90}{33.98±4.69            } & \rotatebox{90}{49.12±3.83      } & \rotatebox{90}{49.12±3.83            } & \rotatebox{90}{29.56±3.21       } & \rotatebox{90}{29.56±3.21                  } & \rotatebox{90}{39.31±2.63  } & \rotatebox{90}{39.31±2.63                  } & \rotatebox{90}{36.23±2.96} & \rotatebox{90}{36.23±2.96              } & \rotatebox{90}{27.15±3.63     } & \rotatebox{90}{27.15±3.63      } & \rotatebox{90}{38.19±4.06       } & \rotatebox{90}{38.19±4.06         } & \rotatebox{90}{39.91±3.29} & \rotatebox{90}{39.91±3.29} & \rotatebox{90}{35.62±1.94            } & \rotatebox{90}{35.62±1.94} & \rotatebox{90}{45.00±5.00             } & \rotatebox{90}{45.00±5.00      } & \rotatebox{90}{27.00±4.46} & \rotatebox{90}{27.00±4.46         } & \rotatebox{90}{36.27±3.37                } & \rotatebox{90}{36.27±3.37} & \rotatebox{90}{42.33±3.88      } & \rotatebox{90}{42.33±3.88      } & \rotatebox{90}{26.19±2.26   } & \rotatebox{90}{26.19±2.26     } & \rotatebox{90}{37.00±4.85} & \rotatebox{90}{37.00±4.85           } & \rotatebox{90}{47.52±2.14} & \rotatebox{90}{47.52±2.14                         } & \rotatebox{90}{43.00±4.98                } & \rotatebox{90}{~~~~~\textbf{34.67}                }\\ \hline
    \rotatebox{90}{\textbf{Full-Finetuning}} & \rotatebox{90}{26.32±4.14            } & \rotatebox{90}{26.32±4.14           } & \rotatebox{90}{31.86±1.89     } & \rotatebox{90}{31.86±1.89       } & \rotatebox{90}{19.85±2.42  } & \rotatebox{90}{19.85±2.42   } & \rotatebox{90}{28.47±3.77        } & \rotatebox{90}{28.47±3.77      } & \rotatebox{90}{27.04±2.71               } & \rotatebox{90}{27.04±2.71     } & \rotatebox{90}{25.18±2.59  } & \rotatebox{90}{25.18±2.59             } & \rotatebox{90}{33.33±4.07} & \rotatebox{90}{33.33±4.07     } & \rotatebox{90}{37.28±2.60           } & \rotatebox{90}{37.28±2.60    } & \rotatebox{90}{35.19±4.62        } & \rotatebox{90}{35.19±4.62         } & \rotatebox{90}{47.26±3.53     } & \rotatebox{90}{47.26±3.53 } & \rotatebox{90}{27.10±2.53             } & \rotatebox{90}{27.10±2.53       } & \rotatebox{90}{38.00±4.88      } & \rotatebox{90}{38.00±4.88            } & \rotatebox{90}{35.00±4.79       } & \rotatebox{90}{35.00±4.79            } & \rotatebox{90}{36.26±3.69      } & \rotatebox{90}{36.26±3.69            } & \rotatebox{90}{27.78±2.31       } & \rotatebox{90}{27.78±2.31                  } & \rotatebox{90}{25.21±2.82  } & \rotatebox{90}{25.21±2.82                  } & \rotatebox{90}{45.45±4.55} & \rotatebox{90}{45.45±4.55              } & \rotatebox{90}{33.01±2.69     } & \rotatebox{90}{33.01±2.69      } & \rotatebox{90}{34.00±4.76       } & \rotatebox{90}{34.00±4.76         } & \rotatebox{90}{16.67±3.33} & \rotatebox{90}{16.67±3.33} & \rotatebox{90}{29.66±3.81            } & \rotatebox{90}{29.66±3.81} & \rotatebox{90}{33.00±4.73             } & \rotatebox{90}{33.00±4.73      } & \rotatebox{90}{33.33±3.07} & \rotatebox{90}{33.33±3.07         } & \rotatebox{90}{28.83±3.56                } & \rotatebox{90}{28.83±3.56} & \rotatebox{90}{32.35±3.28      } & \rotatebox{90}{32.35±3.28      } & \rotatebox{90}{27.27±4.27   } & \rotatebox{90}{27.27±4.27     } & \rotatebox{90}{41.13±3.03} & \rotatebox{90}{41.13±3.03           } & \rotatebox{90}{24.86±3.30} & \rotatebox{90}{24.86±3.30                         } & \rotatebox{90}{31.94±3.18                } & \rotatebox{90}{~~~~~~~\textbf{32.37\dec{-6.63\%}}                } \\ \hline
    \rotatebox{90}{\textbf{Alpaca-LoRA}    } & \rotatebox{90}{33.33±3.31            } & \rotatebox{90}{33.33±3.31           } & \rotatebox{90}{27.00±4.46     } & \rotatebox{90}{27.00±4.46       } & \rotatebox{90}{29.00±4.56  } & \rotatebox{90}{29.00±4.56   } & \rotatebox{90}{32.73±3.66        } & \rotatebox{90}{32.73±3.66      } & \rotatebox{90}{40.08±3.19               } & \rotatebox{90}{40.08±3.19     } & \rotatebox{90}{32.48±2.66  } & \rotatebox{90}{32.48±2.66             } & \rotatebox{90}{38.86±3.52} & \rotatebox{90}{38.86±3.52     } & \rotatebox{90}{24.07±2.61           } & \rotatebox{90}{24.07±2.61    } & \rotatebox{90}{32.95±3.58        } & \rotatebox{90}{32.95±3.58         } & \rotatebox{90}{33.83±3.35     } & \rotatebox{90}{33.83±3.35 } & \rotatebox{90}{32.84±1.90             } & \rotatebox{90}{32.84±1.90       } & \rotatebox{90}{30.92±3.76      } & \rotatebox{90}{30.92±3.76            } & \rotatebox{90}{31.00±4.65       } & \rotatebox{90}{31.00±4.65            } & \rotatebox{90}{25.18±2.59      } & \rotatebox{90}{25.18±2.59            } & \rotatebox{90}{35.32±3.12       } & \rotatebox{90}{35.32±3.12                  } & \rotatebox{90}{44.85±3.02  } & \rotatebox{90}{44.85±3.02                  } & \rotatebox{90}{39.16±3.80} & \rotatebox{90}{39.16±3.80              } & \rotatebox{90}{36.36±4.61     } & \rotatebox{90}{36.36±4.61      } & \rotatebox{90}{39.91±3.29       } & \rotatebox{90}{39.91±3.29         } & \rotatebox{90}{36.11±4.64} & \rotatebox{90}{36.11±4.64} & \rotatebox{90}{23.18±3.45            } & \rotatebox{90}{23.18±3.45} & \rotatebox{90}{30.56±3.85             } & \rotatebox{90}{30.56±3.85      } & \rotatebox{90}{19.61±3.95} & \rotatebox{90}{19.61±3.95         } & \rotatebox{90}{33.53±2.54                } & \rotatebox{90}{33.53±2.54} & \rotatebox{90}{34.82±4.52      } & \rotatebox{90}{34.82±4.52      } & \rotatebox{90}{28.84±2.33   } & \rotatebox{90}{28.84±2.33     } & \rotatebox{90}{38.49±2.99} & \rotatebox{90}{38.49±2.99           } & \rotatebox{90}{35.00±4.79} & \rotatebox{90}{35.00±4.79                         } & \rotatebox{90}{38.72±2.09                } & \rotatebox{90}{~~~~~~~\textbf{33.11\dec{-4.49\%}}                }\\ \hline
    \rotatebox{90}{\textbf{LLaMA-Adapter}  } & \rotatebox{90}{31.61±2.65            } & \rotatebox{90}{31.61±2.65           } & \rotatebox{90}{39.62±3.01     } & \rotatebox{90}{39.62±3.01       } & \rotatebox{90}{30.00±4.61  } & \rotatebox{90}{30.00±4.61   } & \rotatebox{90}{24.82±2.58        } & \rotatebox{90}{24.82±2.58      } & \rotatebox{90}{24.49±2.75               } & \rotatebox{90}{24.49±2.75     } & \rotatebox{90}{32.53±3.65  } & \rotatebox{90}{32.53±3.65             } & \rotatebox{90}{32.32±3.33} & \rotatebox{90}{32.32±3.33     } & \rotatebox{90}{24.51±4.28           } & \rotatebox{90}{24.51±4.28    } & \rotatebox{90}{44.87±3.26        } & \rotatebox{90}{44.87±3.26         } & \rotatebox{90}{24.25±1.43     } & \rotatebox{90}{24.25±1.43 } & \rotatebox{90}{32.73±3.66             } & \rotatebox{90}{32.73±3.66       } & \rotatebox{90}{35.71±4.55      } & \rotatebox{90}{35.71±4.55            } & \rotatebox{90}{37.00±4.85       } & \rotatebox{90}{37.00±4.85            } & \rotatebox{90}{38.30±3.18      } & \rotatebox{90}{38.30±3.18            } & \rotatebox{90}{27.19±4.19       } & \rotatebox{90}{27.19±4.19                  } & \rotatebox{90}{28.29±3.67  } & \rotatebox{90}{28.29±3.67                  } & \rotatebox{90}{24.07±2.61} & \rotatebox{90}{24.07±2.61              } & \rotatebox{90}{28.00±4.51     } & \rotatebox{90}{28.00±4.51      } & \rotatebox{90}{46.78±3.83       } & \rotatebox{90}{46.78±3.83         } & \rotatebox{90}{37.04±4.67} & \rotatebox{90}{37.04±4.67} & \rotatebox{90}{21.76±2.81            } & \rotatebox{90}{21.76±2.81} & \rotatebox{90}{30.23±1.86             } & \rotatebox{90}{30.23±1.86      } & \rotatebox{90}{44.00±4.99} & \rotatebox{90}{44.00±4.99         } & \rotatebox{90}{29.00±4.56                } & \rotatebox{90}{29.00±4.56} & \rotatebox{90}{42.15±1.77      } & \rotatebox{90}{42.15±1.77      } & \rotatebox{90}{36.89±4.78   } & \rotatebox{90}{36.89±4.78     } & \rotatebox{90}{40.00±4.23} & \rotatebox{90}{40.00±4.23           } & \rotatebox{90}{26.00±4.41} & \rotatebox{90}{26.00±4.41                         } & \rotatebox{90}{41.00±4.94                } & \rotatebox{90}{~~~~~~~\textbf{33.62\dec{-3.02\%}}                }\\ \hline
    \rowcolor{Graya} 
    \rotatebox{90}{\textbf{LLaMA-Excitor}  } & \rotatebox{90}{50.43±3.28            } & \rotatebox{90}{50.43±3.28           } & \rotatebox{90}{41.26±3.30     } & \rotatebox{90}{41.26±3.30       } & \rotatebox{90}{40.00±3.02  } & \rotatebox{90}{40.00±3.02   } & \rotatebox{90}{28.43±4.49        } & \rotatebox{90}{28.43±4.49      } & \rotatebox{90}{37.00±4.85               } & \rotatebox{90}{37.00±4.85     } & \rotatebox{90}{40.00±2.79  } & \rotatebox{90}{40.00±2.79             } & \rotatebox{90}{45.87±2.14} & \rotatebox{90}{45.87±2.14     } & \rotatebox{90}{34.31±3.33           } & \rotatebox{90}{34.31±3.33    } & \rotatebox{90}{38.89±3.47        } & \rotatebox{90}{38.89±3.47         } & \rotatebox{90}{27.04±2.71     } & \rotatebox{90}{27.04±2.71 } & \rotatebox{90}{28.16±2.88             } & \rotatebox{90}{28.16±2.88       } & \rotatebox{90}{30.46±3.76      } & \rotatebox{90}{30.46±3.76            } & \rotatebox{90}{42.00±4.96       } & \rotatebox{90}{42.00±4.96            } & \rotatebox{90}{30.00±4.61      } & \rotatebox{90}{30.00±4.61            } & \rotatebox{90}{48.54±3.83       } & \rotatebox{90}{48.54±3.83                  } & \rotatebox{90}{24.25±1.43  } & \rotatebox{90}{24.25±1.43                  } & \rotatebox{90}{30.00±4.61} & \rotatebox{90}{30.00±4.61              } & \rotatebox{90}{25.40±2.24     } & \rotatebox{90}{25.40±2.24      } & \rotatebox{90}{25.46±2.97       } & \rotatebox{90}{25.46±2.97         } & \rotatebox{90}{46.28±4.55} & \rotatebox{90}{46.28±4.55} & \rotatebox{90}{28.55±1.15            } & \rotatebox{90}{28.55±1.15} & \rotatebox{90}{27.59±3.72             } & \rotatebox{90}{27.59±3.72      } & \rotatebox{90}{33.00±4.73} & \rotatebox{90}{33.00±4.73         } & \rotatebox{90}{36.18±3.91                } & \rotatebox{90}{36.18±3.91} & \rotatebox{90}{36.42±3.67      } & \rotatebox{90}{36.42±3.67      } & \rotatebox{90}{37.42±3.80   } & \rotatebox{90}{37.42±3.80     } & \rotatebox{90}{46.00±5.01} & \rotatebox{90}{46.00±5.01           } & \rotatebox{90}{44.00±4.99} & \rotatebox{90}{44.00±4.99                         } & \rotatebox{90}{35.29±1.93                } & \rotatebox{90}{~~~~~~~\textbf{35.75\inc{+3.12\%}}                }\\ \hline         
\end{tabular}

}
\caption{Performances on Massive Multitask Language Understanding tasks (MMLU) under the 5-shot in-context-learning setting.}
\label{tabel:MMLU}
\end{table*}
